Temporal Gains, Spatial Costs: Revisiting Video Fine-Tuning in Multimodal Large Language Models

Multimodal large language models (MLLMs) are typically trained in multiple stages, with video-based supervised fine-tuning (Video-SFT) serving as a key step for improving visual understanding. Yet its effect on the fine-grained evolution of visual capabilities, particularly the balance between spatial and temporal understanding, remains poorly understood. In this paper, we systematically study how Video-SFT reshapes visual capabilities in MLLMs. Across architectures, parameter scales, and frame sampling settings, we observe a consistent pattern: Video-SFT reliably improves video performance, but often yields limited gains or even degradation on static image benchmarks. We further show that this trade-off is closely tied to temporal budget: increasing the number of sampled frames generally improves video performance, but does not reliably improve static image performance. Motivated by this finding, we study an instruction-aware Hybrid-Frame strategy that adaptively allocates frame counts and partially mitigates the image-video trade-off. Our results indicate that Video-SFT is not a free lunch for MLLMs, and preserving spatial understanding remains a central challenge in joint image-video training.

==> figures/R_attention_map.tex <==
\begin{figure}[htbp]
  \centering
  \vspace{-4mm}
  \includegraphics[
  width=1\linewidth,
]{figures/assets/R_attention_map.pdf}

  % \includegraphics[width=1\linewidth]{figures/assets/R_attention_map.pdf}

  % \begin{tikzpicture}
  %       \draw[gray!60, thick] (0,0) rectangle (8,5);  
  %       \draw[gray!60, thick] (0,0) -- (8,5);          
  %       \draw[gray!60, thick] (0,5) -- (8,0);          
  %       \node at (4,2.5) {\Large \textbf{Figure Placeholder}};
  %   \end{tikzpicture}
    \caption{\textbf{Cross-scale attention visualizations}}
      % \vspace{-3mm}
  
  \label{fig:R_attation_map}

\end{figure}

==> sections/old_3_method.tex <==

\section{The Phenomenon: The Temporal Trap behind Visual Modality Conflict}
\label{sec:3_the_phennomenon}
% 本节介绍我们的主要结果和发现。首先，我们进行了一系列受控实验，系统地解析视频级指令微调导致静态视觉理解能力的退化这一现象。这些研究考察了模型的架构（3.1 节）、模型的参数量（3.2节）、训练帧数（3.3 节）这些基本变量的影响。基于这些实验产生的大量数据，我们进一步讨论了视频级指令微调对不同视觉任务的影响。每个小节详细介绍其具体的实验设置或分析方法，随后呈现结果和关键发现。

% fig:3_model_size
% This section is dedicated to presenting our core experimental results and key findings.     We commence by designing and executing a series of controlled experiments to systematically dissect the phenomenon where Video-SFT leads to a performance degradation in the model's static visual comprehension capabilities.     These investigations focus on evaluating the influence of several fundamental variables: the model architecture (Section~\ref{sec:3.1 model architecture}), the model scale (Section~\ref{sec:3.2 model size}).  Based on the substantial data generated from these systematic studies, we further delve into analyzing the effects of Video-SFT  on various downstream vision tasks.     Each subsequent section will elaborate on the specific experimental setups and analytical methodologies employed, followed by the presentation of the corresponding results and observations.

This section introduces an empirical phenomenon we observe in unified image--video MLLMs: Video-SFT improves video comprehension but often leads to stagnation or degradation on static image benchmarks. We term this phenomenon the temporal trap.
We systematically validate that it is not an isolated artifact by evaluating it along three axes: architecture (Sec.~\ref{sec:3.1 model architecture}), scale (Sec.~\ref{sec:3.2 model size}), and fine-grained task categories (Sec.~\ref{sec:3.3 visual tasks}).



\paragraph{Datasets}Our training data is derived from the LLaVA-Next-Video-178k dataset~\cite{zhang2024videoinstructiontuningsynthetic}. 
% We randomly sample 20,000 videos, encompassing a diverse range of video durations (short, medium, and long), to construct a dedicated Video-SFT dataset comprising video-text inputs.
We collect videos from 10 different sources and curate a dataset of 20,000 videos covering various instruction and task formats, including textual descriptions, open-ended questions, and multiple-choice questions. The videos span a wide range of durations (short, medium, and long), ensuring substantial diversity in both content and temporal scale. Based on these data, we constructed a dedicated video-SFT dataset with paired video-text inputs for supervised fine-tuning. Training data statistics are reported in the supplement.
To comprehensively assess and analyze the visual comprehension capabilities of the MLLMs before and after Video-SFT, we selected commonly used benchmarks in recent MLLM literature for both image and video tasks. Specifically, the image benchmarks include MME~\cite{fu2023mme}, MMStar~\cite{chen2024we}, MMBench~\cite{liu2024mmbench}, and POPE~\cite{Li-hallucination-2023}, while the video benchmarks consist of Video-MME~\cite{fu2025video}, MVBench~\cite{li2025mvbench}, TempCompass~\cite{liu2024tempcompass}, and Video-MMMU~\cite{hu2025video}.

% fig:4_train_frame
\input{figures/4_train_frame}

\paragraph{Experimental Setting}
% 对于 MLLMs, 根据视觉编码器和LLM的冻结情况，分为不同的 Instruction tuning strategy。鉴于诸多相关的研究（qwen，llava），我们选择保持视觉编码器冻结的情况下，使用视频指令调优数据对 LLM 进行微调，每组实验超参数保持一致。
The Instruction Tuning Strategy for MLLMs is typically categorized based on the freezing status of the Visual Encoder and the LLM. Consistent with the prevalent studies (\eg Qwen2.5-VL~\cite{bai2025qwen2}, LLaVA~\cite{liu2023visual}), we adopt a specific strategy: the Visual Encoder is kept frozen, and only the LLM is fine-tuned using video instruction tuning data.   We ensure that hyperparameters remain consistent across all experimental groups.

% 我们的训练数据基于LLaVA-Next-Video-178k数据集，随机采样20000个视频，涵盖短、中、长不同时长，构建只包含视频-文本输入的视频指令调优数据。为了综合评估和分析MLLMs的视觉能力，针对图像和视频两类任务，我们分别选取近期 MLLMs 研究中常用的Benchmark：图像Benchmark使用 MME、MMStar、MMBench、POPE，视频Benchmark使用 Video-MME, MVBench，TempCompass, Video-MMMU。


\subsection{Impact of Model Architecture.}
\label{sec:3.1 model architecture}
\findingz{1}{Video-SFT enhances video comprehension but consistently weakens static visual reasoning across architectures.} % Mixed-modality pre-training alleviates but does not eliminate this degradation, revealing an intrinsic conflict between spatial and temporal learning within current MLLMs.

% 我们首先在不同模型架构上探究视频级指令微调对MLLM在静态视觉推理任务上的影响。对目前主流的多模态大语言模型，如Qwen2.5-VL、LLaVA-Next-Video、LLaVA-1.5，我们统一采用均匀采样8帧进行指令微调和评测。我们将微调前后的模型分别在静态图像基准和视频基准上进行评估。

We first investigate the influence of Video-SFT on different architecture models' performance in visual tasks.  We selected several common MLLMs, including Qwen2.5-VL~\cite{bai2025qwen2}, LLaVA-Next-Video~\cite{zhang2024llavanextvideo}, and LLaVA-1.5~\cite{liu2024improved}, and employed the strategy of uniformly sampling 8 frames for both Video-SFT and video benchmarks evaluation.    We conducted a quantitative evaluation of the models before and after Video-SFT on both static image benchmarks and video benchmarks.

% 如图x所示，视频级指令微调确实会导致静态视觉推理的退化。经过视频数据SFT之后，在视频基准上，几乎所有模型的整体准确率均得到提升，这表明我们的微调是有效的，模型确实从训练中有效地学习到了视频理解能力；同时在图像基准上，大部分模型的性能表现出不同程度的下降。从早期MLLM的迭代版本（如LLaVA系列）到最近的模型（如Qwen系列），该现象均广泛存在。这证明了当多模态大语言模型从图像训练阶段过渡到视频阶段时，其在前一阶段学到的视觉理解能力会被削弱或者遗忘。

% \input{figures/1_existing_post_training}

As illustrated in Figure~\ref{fig:3_base_results}, Video-SFT indeed leads to a degradation in model's static visual capabilities.    Following Video-SFT, the overall accuracy of virtually all models on the video benchmarks exhibits an improvement. This strongly validates the efficacy of our Video-SFT, confirming that the models successfully acquired video understanding capabilities. Concurrently, the performance of most models shows varying degrees of decline on the image benchmarks.  This phenomenon is widespread, persisting from early MLLM iterations, such as the LLaVA series, to the latest models, such as the Qwen series. This finding explicitly confirms that the static visual understanding capabilities acquired in the preceding image training phase are attenuated or catastrophically forgotten as the MLLM transitions to Video-SFT phase.

% 仔细观察不同架构的模型，对于没有经过视频数据预训练的LLaVA-1.5，图像和视频任务的变化幅度最大，LLaVA-Next-Video次之，Qwen2.5-VL的变化幅度最小。这说明混合图片和视频数据进行预训练可以在一定程度上缓解这种现象。Qwen2.5-VL，我们推测得益于其M-ROPE机制，使得模型可以同时捕捉和整合一维文本序列、二维视觉图像以及三维视频的位置信息，从而得到进一步改善。但这些方法都没有彻底解决这一现象。

A closer observation of the models across different architectures reveals that LLaVA-1.5~\cite{liu2024improved}, which was not pre-trained on video data, exhibits the largest change in performance across both image and video tasks.   LLaVA-Next-Video shows the second-largest change, while Qwen2.5-VL shows the minimum degradation.  This suggests that pre-training with a mixture of image and video data can partially alleviate temporal trap under visual modality conflict.  For Qwen2.5-VL, perhaps due to its unique M-ROPE mechanism, which allows the model to simultaneously capture and integrate the positional information of 1D text sequences, 2D visual images, and 3D videos, thereby achieving better alignment of modality.  Nevertheless, it is crucial to note that none of these existing approaches completely resolve this temporal trap question. 

% 发现1：


% Mixed-modality pre-training alleviates but does not eliminate this degradation, revealing an intrinsic conflict between spatial and temporal learning within current MLLMs.

% \noindent\textbf{Observation 1.} \textit{\textbf{Video-SFT enhances video comprehension but consistently weakens static visual reasoning across architectures.} Mixed-modality pre-training alleviates but does not eliminate this degradation, revealing an intrinsic conflict between spatial and temporal learning within current MLLMs.}

% fig:3_subTask
\input{figures/3_subTask}

\subsection{Impact of Model Size}
\label{sec:3.2 model size}

% 发现2：模型大小对Video SFT在视频基准上结果的影响较为明显。增加模型大小可以减轻视频级指令调优对静态视觉能力的负面影响。
\findingz{2}{The impact of model size on the results of Video-SFT on the image benchmark is relatively obvious. Increasing the model size can mitigate the effect of Video-SFT on static visual capabilities.} 


% 在分析了模型架构影响之后，我们现在将分析重点转向模型的参数量。为此，我们进行了一系列实验，指令微调了4个不同规模的 Qwen2.5-VL 模型（参数量分别为 3B、7B、32B 和 72B）。每个规模的模型统一采用均匀采样8帧进行训练和评测。

Having systematically analyzed the effect of model architecture, we shift our focus to the influence of model scale. We perform Video-SFT on 4 different sizes of the Qwen2.5-VL model, with parameter sizes of 3B, 7B, 32B, and 72B, respectively. A uniform strategy of uniformly sampling 8 frames was maintained for both training and video benchmarks evaluation across all model scales.

% 如图x所示，对于不同参数量的模型，基本符合“经过视频数据指令微调后，在视频任务上性能上升，而在图像任务上性能下降”这一现象，且随着模型参数量的增加，微调前后呈现出相似的变化趋势。然而，值得注意的是，3B大小的模型的性能显示出异常的变化。对于图片Benchmark，除MME数据集外，3B大小的模型经过视频数据微调后在图像任务上性能均得到一定提升，这可能因为xxxxx

As depicted in Figure~\ref{fig:3_model_size}, the performance of models with varying parameter sizes largely adheres to the general trend of ``performance improvement on video tasks concurrent with a decline on image tasks following video instruction tuning."   Furthermore, the change trend before and after fine-tuning exhibits similarity as the model scale increases.   However, the 3B model shows an anomalous variation in its performance.  Specifically, on image benchmarks, the 3B model's performance on image tasks achieves a certain degree of improvement after video fine-tuning, with the exception of the MME dataset. 

% 对比 7B、32B、72B 大小的模型在指令微调前后的性能变化，随着模型参数量的增加，较大参数量的模型（如72B）性能在不同数据集间展现出一致性，即在图片任务上，模型微调前后的性能差距缩小，甚至反超。这表明较大的模型规模有助于缓解视频级指令微调所导致的静态视觉能力退化。

Compare the performance changes of the 7B, 32B, and 72B models before and after instruction tuning, we observe that as model scale increases, models exhibit high consistency across diverse datasets,  models trained by Video-SFT consistently catch up and surpass base models. This finding indicates that a larger model scale can effectively mitigate the degradation of static visual capabilities caused by video-level instruction tuning.

This finding indicates that a larger model scale can effectively, though partially, mitigate the degradation of static visual capabilities caused by video-level instruction tuning. To further investigate this mechanism, we visualize the cross-scale attention map distributions (see Figure~\ref{fig:R_attation_map}). As shown in the visualizations, when responding to static queries (e.g., "Is there a bird in the image?"), the larger Qwen2.5-VL-72B model successfully maintains localized spatial focus on the key object after Video-SFT. In contrast, smaller models (e.g., 7B and 32B) exhibit highly dispersed attention maps, indicating that their spatial alignment is more easily disrupted by temporal bias.

\input{figures/R_attention_map}

% table2_mix_frame_table



% \noindent\textbf{Observation 2.} \textit{\textbf{The impact of model size on the results of Video-SFT on the image benchmark is relatively obvious.} Increasing the model size can mitigate the effect of video-level instruction tuning on static visual capabilities.}

\subsection{Impact of Video-SFT cross Visual Tasks}
\label{sec:3.3 visual tasks}

% 基于第3节的实验结果，我们基本证实了“视频级指令微调确实会导致静态视觉推理”这一现象在不同架构和规模的模型上都普遍存在。现在，我们将之前的研究结果进行综合，以探究视觉任务的内部变化。视频级指令微调导致静态视觉推理能力退化，是一种单一的、统一的影响，还是对于不同的视觉任务有所差别？ 为了回答这个问题，我们将视觉任务进一步细化，划分为感知、推理和幻觉（幻觉不知道能不能单独算一个）三种类别。具体而言，对于MME、MMStar和MMBench三个通用数据集，我们将其子任务划分为感知和推理两个大类，其中感知任务又可以分为细粒度和粗粒度两个维度，同时，使用POPE数据集专门评测幻觉任务。

Building upon the experimental results in Sections~\ref{sec:3.1 model architecture}, we have generally confirmed the pervasiveness of the phenomenon where "video-level instruction tuning leads to the degradation of static visual reasoning capabilities" across various model architectures and scales. We now synthesize the findings from Sections~\ref{sec:3_the_phennomenon} to delve into the impact of video-level instruction tuning on the changes within internal visual tasks. A central question is whether the degradation of static visual reasoning capabilities caused by video instruction tuning is a singular, uniform effect or if it exhibits a differentiated impact across distinct categories of visual tasks. 

\input{tables/4_mix_frame_table}

To address this, we further refine the visual tasks into three major categories: Perception, Reasoning, and Hallucination. Specifically, for the general benchmarks MME, MMStar, and MMBench, we categorize their sub-tasks into Perception and Reasoning groups, and specifically utilize the POPE dataset to evaluate Hallucination Suppression Capability.

% 如图5所示，以3.1节中Qwen2.5-VL-7B模型Video-SFT前后子啊MME, MMStar 和 MMBench 数据集上的性能变化为例, 我们进一步展示了更为细化的子任务。我们分析3.1节中的实验数据，得到了4个统计性结果：（1）经过Video-SFT，模型在感知任务上性能下降最大，而推理性任务性能下降适中。（2）在感知任务中，Video-SFT后模型在细粒度感知任务上的性能下降程度高于粗粒度感知任务（3）在推理任务中，数学相关的推理任务性能总体得到提升。

Based on the experimental results in Section~\ref{sec:3.1 model architecture}, we further statistically analyzed the performance variation of different models on the image benchmarks, which reveals the following critical observations: (1) Training with video data results in the maximum degradation in performance for Perception tasks, while the decline in Reasoning tasks is comparatively moderate.  (2) Within Perception tasks, the model's performance on fine-grained perception degrades substantially greater than that on coarse-grained perception. (3) Among Reasoning tasks, the performance on math-related reasoning tasks is generally improved.





==> sections/old_4_experimental.tex <==
\section{Exploration}


% \input{tables/4_mix_16f_table}

\subsection{Impact of Fine-tuning Frame Count.}
\label{sec:4.1 train frame}

\findingz{3}{The improvement effect of the training frame count on model performance has an upper limit, showing a tendency toward saturation or decline after reaching a critical point.}
%This reveals the existence of redundant temporal information and the temporal trap phenomenon, which harms the model's generalization capability for visual features.

% 接下来，我们专注于指令微调本身，探索使用图像和视频数据进行训练本质上的不同——帧数。我们使用不同的帧采样策略对 Qwen2.5-VL-7B 模型进行指令微调，即将视频分别均匀采样 8帧、16帧、32帧、64帧 作为输入数据。

We now focus on the instruction tuning process itself to explore a fundamental distinction between training with image versus video data, namely, the number of frames.   To this end, we conducted instruction tuning on the Qwen2.5-VL-7B model using different frame sampling strategies, where videos were uniformly sampled with 8, 16, 32 and 64 frames to serve as the input data.

% 如图4所示，随着模型训练时采样帧数的增加，下游的视觉任务性能普遍得到提升。然而，观察两种视觉任务，可以发现显著的差别。视频任务对帧数的敏感度远高于图像任务，所有的视频Benchmark都呈现出相似的趋势，随采样帧数的增加而持续提升。与之形成鲜明对比的是，图像Benchmark的准确率随帧数变化幅度较小，且变化趋势存在起伏。

As depicted in Figure~\ref{fig:3_train_frame}, performance on the downstream visual tasks generally improves with the increase in the number of sampled frames during model training. However, a significant discrepancy is observed when comparing the two types of visual tasks: video tasks exhibit a much higher sensitivity to frame count than image tasks. All video benchmarks demonstrate a similar trend, with performance consistently improving as the sampled frame count increases. In stark contrast, the accuracy on image benchmarks shows a smaller magnitude of change and fluctuations with varying frame counts. 

% 具体而言，观察视频基准的性能变化，可以发现，随着训练帧数从 8 增加到 64，模型的准确率持续且显著地提升，这证实了时间信息对视频理解的重要性。然而，性能的提升速率均随帧数的增加明显放缓，呈现出边际效用递减的趋势。这表明即使对于视频任务，更多的帧数，亦或者说更多的时间信息虽然有益，但在到达某一阈值之后，额外增加的帧数所带来的性能增益将不再与计算成本成正比。

Specifically, by observing the performance on video benchmarks, we find that the model's accuracy sustainedly and significantly improves as the training frame count increases from 8 to 64, which validates the importance of temporal information for video comprehension.  However, the performance gain rate evidently decelerates with the increase in frame count, exhibiting a trend of diminishing marginal returns.  This suggests that although more frames (more temporal information) are beneficial for video tasks, the performance gain provided by additional frames beyond a certain threshold is no longer commensurate with the computational overhead.

% 对于图像基准，呈现出更加明显的变化。随着训练帧数的不断增加，图像基准如MMStar呈现出于视频基准类似的提升速率放缓的趋势。MMBench和POPE的准确率甚至出现先上升后下降的现象。这明确地表明，帧数，即时间信息并非越多越好，训练时过多冗余的时间信息反而让模型产生结构偏差，从而损害了静态图像表示的对齐和泛化，即“时间陷阱”现象。
For image benchmarks, a more pronounced variation is observed.   As the training frame count continuously increases, image benchmarks such as MMStar display a similar trend of performance gain  rate as seen in video benchmarks.   However, the accuracy for MMBench and POPE exhibits an initial increase followed by a decline.   This explicitly highlights that an increased frame count (more temporal information), is not always beneficial;   excessive redundant temporal information during training may induce a structural bias in the model, thereby damaging the alignment and generalization of static image representations—a phenomenon we term the temporal trap.

\subsection{Hybrid-Frame Strategy}
\label{sec:4.2 Hybrid-Frame Strategy}

% 4.1节的现象引发了我们的思考，能否引入一种混合帧的训练策略，根据每条指令的时空依赖程度自适应地确定输入帧的数量，而不是均匀采样或根据视频时长采样，从而缓解时间陷阱问题。

The phenomenon in Section~\ref{sec:4.1 train frame} provokes our reflection on introducing a Hybrid-Frame Strategy that adaptively determines the number of input frames based on the spatiotemporal dependency of each instruction, instead of uniformly sampling frames based solely on video duration, in order to mitigate Temporal Trap problem.

% 具体来说， 我们利用 Qwen3-VL 模型在多模态任务上的卓越性能 ，对每条指令进行时间和空间维度的综合评估 。然后，模型预测解析指令查询所需的最合适的帧数 ，随后将其用作相应视频的采样帧数 。

% Specifically, leveraging the superior performance of the Qwen3-VL model on multimodal tasks, we subject each instruction to a comprehensive evaluation across both temporal and spatial dimensions. The model then predicts the most appropriate number of frames required to complete the instruction, which is subsequently used as the sampling frame count for the corresponding video.

Specifically, leveraging the strong multimodal capability of the Qwen3-VL model, we formulate the estimation of the required frame number as an instruction-aware spatiotemporal analysis task. For each training sample, the model performs a holistic assessment of both temporal and spatial dependencies, determining how much temporal evidence and what degree of spatial granularity are necessary for faithfully solving the instruction. Concretely, given an instruction $I$ and its paired video $V$, Qwen3-VL is prompted to evaluate aspects such as event duration, motion continuity, causal relations, object interactions, and fine-grained visual attributes, and outputs an instruction-specific frame count $\hat{n}$. This process can be viewed as a regression-style prediction task, where the model adaptively infers the optimal number of frames required for the downstream query.
% 我们使用该方法对训练集的每一条数据进行了评估，使用得到的帧数作为训练时的采样帧数，对Qwen2.5-VL-7B进行Video-SFT，平均训练帧数为11帧，其他条件与4.1节中的实验保持一致。帧数的具体分布情况见附录x。(均匀采样8帧进行视频基准的评测。）

We employed this method to evaluate every sample in the training set.  The resulting frame counts were then used as the sampling frame count for the Video-SFT of Qwen2.5-VL-7B.  The average training frame count was 11 frames, while all other experimental conditions remained consistent with Section~\ref{sec:4.1 train frame}.  The detailed distribution of the frame counts is presented in Appendix.
Our goal with this strategy is not necessarily to surpass every fixed-frame configuration on all metrics, but to effectively mitigate the temporal trap at a much lower training cost. By dynamically allocating frames, the model can "cover" necessary temporal evidence without being overwhelmed by redundant frames.

To validate the necessity of using an MLLM for instruction-aware frame allocation, we evaluated two alternative frame-sampling variants: (i) a heuristic approach selecting frames based on inter-frame similarity computed from DINOv2, and (ii) using a smaller VLM (Qwen2.5-VL-3B) as the frame-count predictor. As shown in Table X, the heuristic DINOv2 method falls short in preserving static image performance, underscoring that simple visual deduplication cannot replace instruction-aware spatiotemporal allocation. Furthermore, while the 7B predictor yields the optimal overall trade-off, the 3B-based predictor still achieves strong and consistent improvements. This demonstrates that utilizing an MLLM for the frame selection strategy is fundamentally necessary and highly effective, even when employing smaller-scale models.
% 实验结果如表2所示。对于图片基准，我们所提出混合帧的训练策略在MMStar和POPE数据集上取得了最高的准确率，超过了使用更多帧数如32、64帧进行训练的模型。同时，相较于基准模型，混合帧策略也有效提高了视频任务的性能。

%[xxxx] 

%这充分说明混合帧策略有效性，在节约训练成本的同时，有效缓解视觉模态冲突下的时序陷阱问题，在图像和视频两种视觉模态之间实现平衡优化。
The experimental results are presented in Table~\ref{tab:video_sft_all}. For the image benchmarks, our proposed Hybrid-Frame Strategy achieves the highest accuracy on the MMStar and POPE datasets, outperforming models trained with a higher fixed frame count, such as 32 or 64 frames. Simultaneously,  Hybrid-Frame Strategy also effectively enhances the performance on video tasks compared to the baseline model. 
% need something

This clearly demonstrates the efficacy of Hybrid-Frame Strategy, which effectively mitigates the temporal trap problem under visual modality conflict while reducing training costs and achieving a balanced optimization between the image and video visual modalities.

To further demonstrate that our strategy generalizes beyond the Qwen architecture, we apply the Hybrid-Frame Strategy to LLaVA-1.5-7B. As shown in Table~\ref{tab:s_llava-1.5-frame}. the strategy yields the best overall image performance across different Video-SFT budgets, confirming that instruction-aware frame allocation is a broadly effective mechanism for mitigating the temporal trap across distinct MLLM architectures.

\input{tables/s_llava_1.5_frame}


\input{tables/4_mix_16f_table.tex}

\input{tables/s_total_model_frame}

% %模型性能随帧数的增加而不断提高，但总体来看，增加训练时采样帧数可以在一定程度上缓解模型经过视频数据训练后在图像Benchmark上性能下降的现象。

% Nevertheless, an overall trend suggests that increasing the frame count during training can partially alleviate the performance degradation phenomenon on image benchmarks following fine-tuning with video data.




==> tables/4_mix_16f_table.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\caption{\textbf{Performance comparison of Qwen2.5-VL-7B under different Video-SFT strategies across multiple frame settings}. 
Numbers in \textcolor{darkgreen}{$\uparrow$} indicate improvements, while numbers in \textcolor{red}{$\downarrow$} indicate degradations relative to the base model under the same frame setting. 
Increasing SFT frame count generally enhances temporal modeling, while our \textbf{Hybrid-Frame Strategy} further boosts performance in most settings.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Setting} & \textbf{Video-MME} & \textbf{Video-MMMU} & \textbf{MVBench} \\
\midrule
\multicolumn{4}{l}{\textbf{8 Frames}} \\
\midrule
Base & 51.19 & 44.22 & 62.68 \\
+ Video-SFT-8F & 54.41 {\color{darkgreen}(↑3.22)} & 47.56 {\color{darkgreen}(↑3.34)} & 64.62 {\color{darkgreen}(↑1.94)} \\
\rowcolor[RGB]{245,248,255}
+ Hybrid-Frame (Ours) & 54.96 {\color{darkgreen}(↑3.77)} & 47.22 {\color{darkgreen}(↑3.00)} & 63.94 {\color{darkgreen}(↑1.26)} \\
\midrule

\multicolumn{4}{l}{\textbf{16 Frames}} \\
\midrule
Base & 55.96 & 48.56 & 64.41 \\
+ Video-SFT-16F & 58.74 {\color{darkgreen}(↑2.78)} & 50.44 {\color{darkgreen}(↑1.88)} & 66.00 {\color{darkgreen}(↑1.59)} \\
\rowcolor[RGB]{245,248,255}
+ Hybrid-Frame (Ours) & 58.15 {\color{darkgreen}(↑2.19)} & 51.78 {\color{darkgreen}(↑3.22)} & 64.55 {\color{darkgreen}(↑0.14)} \\
\midrule

\multicolumn{4}{l}{\textbf{32 Frames}} \\
\midrule
Base & 60.07 & 49.67 & 66.45 \\
+ Video-SFT-32F & 61.30 {\color{darkgreen}(↑1.23)} & 51.44 {\color{darkgreen}(↑1.77)} & 66.51 {\color{darkgreen}(↑0.06)} \\
\rowcolor[RGB]{245,248,255}
+ Hybrid-Frame (Ours) & 61.52 {\color{darkgreen}(↑1.45)} & 55.12 {\color{darkgreen}(↑5.45)} & 63.38 {\color{red}(↓3.07)} \\
\midrule

\multicolumn{4}{l}{\textbf{64 Frames}} \\
\midrule
Base & 61.67 & 49.78 & 67.92 \\
+ Video-SFT-64F & 61.93 {\color{darkgreen}(↑0.26)} & 51.44 {\color{darkgreen}(↑1.66)} & 66.89 {\color{red}(↓1.03)} \\
\rowcolor[RGB]{245,248,255}
+ Hybrid-Frame (Ours) & 60.93 {\color{red}(↓0.74)} & 55.91 {\color{darkgreen}(↑6.13)} & 68.57 {\color{darkgreen}(↑0.65)} \\
\bottomrule
\end{tabular}
}

\label{tab:video_sft_all}
\vspace{-10pt}
\end{table}


==> tables/4_mix_frame_table.tex <==
\begin{table}
\centering
\small
\caption{\textbf{Performance comparison of Qwen2.5-VL-7B under different Video-SFT strategies on image benchmarks only.}
Numbers in \textcolor{darkgreen}{$\uparrow$} indicate improvements, while numbers in \textcolor{red}{$\downarrow$} indicate degradations relative to the base model.
Although increasing video-frame SFT helps temporal modeling, it often harms static visual capability, whereas our \textbf{Hybrid-Frame Strategy} preserves and improves image understanding.}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{} 
& \multicolumn{2}{c}{\textbf{Image Benchmark}} \\
\cmidrule(lr){2-3}
& MMStar & POPE \\
\midrule
\textbf{Qwen2.5-VL-7B (Base)} 
& 62.07 & 88.03 \\
\midrule

\textbf{+ Video-SFT-8F} 
& 61.67 {\color{red}(↓0.40)} 
& 87.82 {\color{red}(↓0.21)} \\

\textbf{+ Video-SFT-16F} 
& 62.00 {\color{red}(↓0.07)} 
& \underline{87.93} {\color{red}(↓0.10)} \\

\textbf{+ Video-SFT-32F} 
& 62.20 {\color{darkgreen}(↑0.13)} 
& \textbf{88.20} {\color{darkgreen}(↑0.17)} \\

\textbf{+ Video-SFT-64F} 
& \underline{62.27} {\color{darkgreen}(↑0.20)} 
& 87.89 {\color{red}(↓0.14)} \\
\midrule

\rowcolor[RGB]{245,248,255}
\textbf{+ Hybrid-Frame Strategy (Ours)}
& \textbf{62.33} {\color{darkgreen}(↑0.26)} 
& \textbf{88.20} {\color{darkgreen}(↑0.17)} \\
\bottomrule
\end{tabular}
}
\label{Table:MixFrameImageOnly}
\end{table}


==> tables/R_hybrid_compare.tex <==

% \setlength{\textfloatsep}{10pt}
\captionsetup[table]{skip=4pt}
\renewcommand{\arraystretch}{0.95}

\begin{table}[h]
  \centering
      \vspace{-2mm}
  \caption{\textbf{Comparison of different method of frame sampling.}}
  \footnotesize
  \resizebox{\columnwidth}{!}{%

    \begin{tabular}{lccccc}
    \toprule
    & \textbf{MMStar} & \textbf{POPE} & \textbf{Video-MME} & \textbf{Video-MMMU} & \textbf{MVBench} \\
    \midrule
\textbf{Base}       
& 62.07 
& 88.03 
& 51.19 
& 44.22 
& 62.28 \\

\textbf{~+ Hybrid-Frame (Ours)}       
& 62.33\textcolor{ForestGreen}{↑} 
& 88.20\textcolor{ForestGreen}{↑} 
& 54.96\textcolor{ForestGreen}{↑} 
& 47.22\textcolor{ForestGreen}{↑} 
& 63.94\textcolor{ForestGreen}{↑} \\

\textbf{~ + Frame-similarity–based}
& \textcolor{red}{61.40↓} 
& \textcolor{red}{87.91↓} 
& 53.96\textcolor{ForestGreen}{↑} 
& 47.13\textcolor{ForestGreen}{↑} 
& 63.14\textcolor{ForestGreen}{↑} \\

\textbf{~ + Qwen2.5-VL-3B-based}        
& 62.19\textcolor{ForestGreen}{↑} 
& 88.19\textcolor{ForestGreen}{↑} 
& 53.47\textcolor{ForestGreen}{↑} 
& 47.91\textcolor{ForestGreen}{↑} 
& 64.25\textcolor{ForestGreen}{↑} \\

    \bottomrule
  \end{tabular}%
  }
        \vspace{-2mm}
  \label{tab:benchmark_results}
\end{table}

  % \begin{tabular}{lcccccc}
  %   \toprule
  %   & MMStar & POPE & mmbench & Video MME & MMMU & MVBench \\
  %   \midrule
  %   base       & 62.07 & 88.03 & 51.19 & 51.19 & 44.22 & 62.28 \\
  %   ours       & 62.33 & 88.20 & 54.96 & 54.96 & 47.22 & 63.94 \\
  %   tradition  & 61.40 & 87.91 & 53.96 & 53.96 & 47.13 & 63.14 \\
  %   3b         & 62.00 & 88.19 & 55.47 & 53.47 & 47.91 & 64.25 \\
  %   \bottomrule
  % \end{tabular}%
  % }


==> tables/R_llava_1.5_frame.tex <==
% \begin{table}[t]
%   \centering
%   \footnotesize
%   \adjustbox{max width=\columnwidth}{%
%   \begin{tabular}{lcccccc}
%     \toprule
%     & MMStar & POPE & mmbench & MME\_Video & MVBench & MMMU \\
%     \midrule
%     Base & 32.93 & 88.69 & 58.51 & 25.67 & 38.39 & 8.67 \\
%     8f   & 28.87 & 71.69 & 37.12 & 38.59 & 44.92 & 18.56 \\
%     16f  & 28.47 & 72.78 & 35.44 & 51.39 & 44.45 & 16.44 \\
%     32f  & 29.40 & 73.40 & 34.10 & 59.90 & 41.09 & 12.92 \\
%     mix  & 32.47 & 75.66 & 54.24 & 52.41 & 43.88 & 18.71 \\
%     \bottomrule
%   \end{tabular}%
%   }
%   \caption{Results under different frame sampling strategies.}
%   \label{tab:fps_results}
% \end{table}

% \setlength{\textfloatsep}{10pt}
\captionsetup[table]{skip=4pt}
\renewcommand{\arraystretch}{0.95}

\begin{table}[h]
  \centering
  \footnotesize
        \vspace{-2mm}
  \caption{\textbf{LLaVA-1.5-7B under different Video-SFT strategies.}}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{lcccccc}
       \toprule
    & \textbf{MMStar} & \textbf{POPE} & \textbf{MMBench} & \textbf{MME-Video} & \textbf{MMMU-Video} \\
    \midrule
\textbf{Base} 
& 32.93 & 88.69 & 58.51 & 25.67  & 8.67 \\

\textbf{+8F}   
& 28.87 
& 71.69 
& \underline{37.12} 
& 38.59 
& \underline{18.56} \\

\textbf{+16F}  
& 28.47 
& 72.78 
& 35.44 
& 51.39 
& 16.44 \\

\textbf{+32F}  
& \underline{29.40} 
& \underline{73.40} 
& 34.10 
& \textbf{59.90} 
& 12.92 \\

\textbf{+Ours}  
& \textbf{32.47} 
& \textbf{75.66} 
& \textbf{54.24} 
& \underline{52.41} 
& \textbf{18.71} \\

    \bottomrule
  \end{tabular}%
  }
  
  \label{tab:llava-1.5-frame}
\end{table}


==> tables/s_llava_1.5_frame.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\caption{\textbf{Performance comparison of LLaVA-1.5-7B under different Video-SFT strategies.}
Increasing the frame count improves video understanding but often degrades image-centric perception. 
Our \textbf{Hybrid-Frame Strategy} provides a better balance between the two.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccc|cc}
\toprule
\multirow{2}{*}{\textbf{Setting}} & \multicolumn{3}{c|}{\textbf{Image Benchmarks}} & \multicolumn{2}{c}{\textbf{Video Benchmarks}} \\
& \textbf{MMStar} & \textbf{POPE} & \textbf{MMBench} & \textbf{MME-Video} & \textbf{MMMU-Video} \\
\midrule
Base 
& 32.93 & 88.69 & 58.51 & 25.67 & 8.67 \\

+ Video-SFT-8F
& 28.87 & 71.69 & \underline{37.12} & 38.59 & \underline{18.56} \\

+ Video-SFT-16F
& 28.47 & 72.78 & 35.44 & 51.39 & 16.44 \\

+ Video-SFT-32F
& \underline{29.40} & \underline{73.40} & 34.10 & \textbf{59.90} & 12.92 \\

\rowcolor[RGB]{245,248,255}
+ Hybrid-Frame (Ours)
& \textbf{32.47} & \textbf{75.66} & \textbf{54.24} & \underline{52.41} & \textbf{18.71} \\
\bottomrule
\end{tabular}
}
\label{tab:s_llava-1.5-frame}
\vspace{-8pt}
\end{table}


==> tables/s_n_images_table.tex <==
\begin{table}[!htbp] 
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \caption{\textbf{Comparison of Qwen2.5-VL-7B model's performance on MME, MMStar and MMBench before and after 8, 16, 32 and 64 frames of Video-SFT, where the number of input images is the same as the number of frames used in Video-SFT.} \textbf{Key Insight:} (1) SFT models generally lag behind Base models for any given number of frames. (2) A greater number of redundant image inputs hurt visual performance for MLLMs, justifying our \textbf{Hybrid-Frame Strategy}.}
    \label{tab:s_n_images_table}
    \begin{tabular}{l|c|ccc}
        \toprule
        \textbf{Model Setting} & \textbf{Frames ($N$)} & \textbf{MME} & \textbf{MMStar} & \textbf{MMBench} \\
        \midrule
        Base Model & 8 & 2360 & 60.20 & 87.83 \\
        \rowcolor{gray!15} Video-SFT & 8 & 2204 & 60.33 & 86.44 \\
        \midrule
        Base Model & 16 & 2342 & 59.73 & 87.36 \\
        \rowcolor{gray!15} Video-SFT & 16 & 2253 & 59.27 & 86.39 \\
        \midrule
        Base Model & 32 & 2286 & 59.33 & 86.90 \\
        \rowcolor{gray!15} Video-SFT & 32 & 2220 & 58.53 & 86.07 \\
        \midrule
        Base Model & 64 & 2272 & 58.00 & 85.74 \\
        \rowcolor{gray!15} Video-SFT & 64 & 2191 & 57.13 & 85.33 \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/table_templates.tex <==
% AAAI
\begin{table}
\centering
\scalebox{0.9}{
\begin{tabular}{lcccc} 
\hline

\hline
\end{tabular}
}
\caption{}
\label{tab:ra_results}
\end{table}
